Generating $SROI^-$ Ontologies via Knowledge Graph Query Embedding Learning

Query embedding approaches answer complex logical queries over incomplete knowledge graphs (KGs) by computing and operating on low-dimensional vector representations of entities, relations, and queries. However, current query embedding models heavily rely on excessively parameterized neural networks and cannot explain the knowledge learned from the graph. We propose a novel query embedding method, AConE, which explains the knowledge learned from the graph in the form of $SROI^-$ description logic axioms while being more parameter-efficient than most existing approaches. AConE associates queries to a $SROI^-$ description logic concept. Every $SROI^-$ concept is embedded as a cone in complex vector space, and each $SROI^-$ relation is embedded as a transformation that rotates and scales cones. We show theoretically that AConE can learn $SROI^-$ axioms, and defines an algebra whose operations correspond one to one to $SROI^-$ description logic concept constructs. Our empirical study on multiple query datasets shows that AConE achieves superior results over previous baselines with fewer parameters. Notably on the WN18RR dataset, AConE achieves significant improvement over baseline models. We provide comprehensive analyses showing that the capability to represent axioms positively impacts the results of query answering.

==> A_Theory_Proof.tex <==
\section{Theory Proof}

\begin{table*}[b]
\caption{AConE's MRR mean values and standard variances ($\%$) on answering tree-form ($\exists$, $\land$, $\lor, \neg$) queries}
\label{EPFOL(sd)}
\centering
%\resizebox{\textwidth}{!}{
\begin{tabular}{lllllllllllllll}
\hline
\textbf{Dataset} & \textbf{1p} & \textbf{2p} & \textbf{3p} & \textbf{2i} & \textbf{3i} & \textbf{pi} & \textbf{ip} & \textbf{2u} & \textbf{up} & \textbf{2in} & \textbf{3in} & \textbf{inp} & \textbf{pin} & \textbf{pni}\\
\hline
$\multirow{2}{5em}{NELL}$ & 54.5$\pm$ & 17.7$\pm$ & 14.4$\pm$ & 41.9$\pm$ & 53.0$\pm$ & 26.1$\pm$ & 20.7$\pm$ & 16.5$\pm$ & 12.8$\pm$ & 5.2$\pm$ & 7.7$\pm$ & 9.4$\pm$ & 3.2$\pm$ & 3.7$\pm$\\
& 0.097 & 0.152 & 0.192 & 0.130 & 0.038 & 0.084 & 0.146 & 0.112 & 0.137& 0.012 & 0.079 & 0.154 & 0.012 & 0.097\\
\hline
\end{tabular}
%}
\end{table*}

\label{Lemmas and Proofs}
\begin{lemma}
AConE can infer symmetry and anti-symmetry patterns. 
\label{lemma1}
\end{lemma}
\begin{proof}
Given cone query embeddings $X = (\mathbf{h}_{U}^{x},\mathbf{h}_{L}^{x})$, $Y = (\mathbf{h}_{U}^{y},\mathbf{h}_{L}^{y})$ and relation $r = (\mathbf{r}_{U},\mathbf{r}_{L})$,
if $(X,r,Y)$ and $(Y,r,X)$ hold, we have
\begin{equation}
\begin{split}
(\mathbf{h}_{U}^{x}\circ\mathbf{r}_{U},\mathbf{h}_{L}^{x}\circ\mathbf{r}_{L}) =(\mathbf{h}_{U}^{y},\mathbf{h}_{L}^{y}),\\
(\mathbf{h}_{U}^{y}\circ\mathbf{r}_{U},\mathbf{h}_{L}^{y}\circ\mathbf{r}_{L}) =(\mathbf{h}_{U}^{x},\mathbf{h}_{L}^{x}),
\end{split}
\end{equation}
\begin{equation}\rightarrow (\mathbf{h}_{U}^{y}\circ\mathbf{r}_{U}\circ\mathbf{r}_{U},\mathbf{h}_{L}^{y}\circ\mathbf{r}_{L}\circ\mathbf{r}_{L})=(\mathbf{h}_{U}^{y},\mathbf{h}_{L}^{y})\end{equation}
thus, it is inferrable that $X$ is symmetric to $Y$ if and only if $(\mathbf{r}_{U}\circ\mathbf{r}_{U} = \mathbf{1},\mathbf{r}_{L}\circ\mathbf{r}_{L} = \mathbf{1})$. Similarly, if $(X,r,Y)$ and $\neg(Y,r,X)$ hold, we have:
\begin{equation}
\begin{split}
(\mathbf{h}_{U}^{x}\circ\mathbf{r}_{U},\mathbf{h}_{L}^{x}\circ\mathbf{r}_{L}) =(\mathbf{h}_{U}^{y},\mathbf{h}_{L}^{y}),\\
(\mathbf{h}_{U}^{y}\circ\mathbf{r}_{U},\mathbf{h}_{L}^{y}\circ\mathbf{r}_{L})\neq(\mathbf{h}_{U}^{x},\mathbf{h}_{L}^{x}),
\end{split}
\end{equation}
\begin{equation}\rightarrow (\mathbf{h}_{U}^{x}\circ\mathbf{r}_{U}\circ\mathbf{r}_{U},\mathbf{h}_{L}^{x}\circ\mathbf{r}_{L}\circ\mathbf{r}_{L})\neq(\mathbf{h}_{U}^{x},\mathbf{h}_{L}^{x})
\end{equation}
thus, it is inferrable that $X$ is anti-symmetric to $Y$ if and only if $(\mathbf{r}_{U}\circ\mathbf{r}_{U} \neq \mathbf{1},\mathbf{r}_{L}\circ\mathbf{r}_{L} \neq \mathbf{1})$. 
\end{proof}
%
\begin{lemma}
AConE can infer  inverse patterns.
\label{lemma2}
\end{lemma}
\begin{proof}
Given cone query embeddings $X = (\mathbf{h}_{U}^{x},\mathbf{h}_{L}^{x})$, $Y = (\mathbf{h}_{U}^{y},\mathbf{h}_{L}^{y})$ and relations $r_{1} = (\mathbf{r}_{U,1},\mathbf{r}_{L,1})$, $r_{2} = (\mathbf{r}_{U,2},\mathbf{r}_{L,2})$
if $(X,r_{1},Y)$ and $(Y,r_{2},X)$ hold, we have
\begin{equation}
\begin{split}
(\mathbf{h}_{U}^{x}\circ\mathbf{r}_{U,1},\mathbf{h}_{L}^{x}\circ\mathbf{r}_{L,1})=(\mathbf{h}_{U}^{y},\mathbf{h}_{L}^{y}),\\
(\mathbf{h}_{U}^{y}\circ\mathbf{r}_{U,2},\mathbf{h}_{L}^{y}\circ\mathbf{r}_{L,2})=(\mathbf{h}_{U}^{x},\mathbf{h}_{L}^{x}),
\end{split}
\end{equation}
\begin{equation}
\rightarrow (\mathbf{h}_{U}^{y}\circ\mathbf{r}_{U,2}\circ\mathbf{r}_{U,1},\mathbf{h}_{L}^{y}\circ\mathbf{r}_{L,2}\circ\mathbf{r}_{L,1})=(\mathbf{h}_{U}^{y},\mathbf{h}_{L}^{y})
\end{equation}
thus, it is inferrable that X is inverse to Y if and only if $\mathbf{r}_{U,2}\circ\mathbf{r}_{U,1}=1$ and $\mathbf{r}_{L,2}\circ\mathbf{r}_{L,1}=1$.
\end{proof}
%
\begin{lemma}
AConE can infer the composition pattern.
\label{lemma3}
\end{lemma}
\begin{proof}
Given cone query embeddings $X = (\mathbf{h}_{U}^{x},\mathbf{h}_{L}^{x})$, $Y = (\mathbf{h}_{U}^{y},\mathbf{h}_{L}^{y})$, $Z = (\mathbf{h}_{U}^{z},\mathbf{h}_{L}^{z})$ and relations $r_{1} = (\mathbf{r}_{U,1},\mathbf{r}_{L,1})$, $r_{2} = (\mathbf{r}_{U,2},\mathbf{r}_{L,2})$,
$r_{3} = (\mathbf{r}_{U,3},\mathbf{r}_{L,3})$,
if $(X,r_{1},Y)$, $(Y,r_{2},Z)$ and $(X,r_{3},Z)$ hold, we have
\begin{equation}
\begin{split}
(\mathbf{h}_{U}^{x}\circ\mathbf{r}_{U,1},\mathbf{h}_{L}^{x}\circ\mathbf{r}_{L,1})=(\mathbf{h}_{U}^{y},\mathbf{h}_{L}^{y}),\\
(\mathbf{h}_{U}^{y}\circ\mathbf{r}_{U,2},\mathbf{h}_{L}^{y}\circ\mathbf{r}_{L,2})=(\mathbf{h}_{U}^{z},\mathbf{h}_{L}^{z}),\\
(\mathbf{h}_{U}^{x}\circ\mathbf{r}_{U,3},\mathbf{h}_{L}^{x}\circ\mathbf{r}_{L,3})=(\mathbf{h}_{U}^{z},\mathbf{h}_{L}^{z}),
\end{split}
\end{equation}
\begin{equation}
\rightarrow
(\mathbf{h}_{U}^{x}\circ\mathbf{r}_{U,1}\circ\mathbf{r}_{U,2},\mathbf{h}_{L}^{x}\circ\mathbf{r}_{L,1}\circ\mathbf{r}_{L,2}) = (\mathbf{h}_{U}^{x}\circ\mathbf{r}_{U,3},\mathbf{h}_{L}^{x}\circ\mathbf{r}_{L,3})
\end{equation}
thus, it is inferrable that relation $r_3$ is compositional of $r_1$ and $r_2$ if and only if $\mathbf{r}_{U,1}\circ\mathbf{r}_{U,2}=\mathbf{r}_{U,3}$.
\end{proof}



\section{Classification Process of Test Queries}
\label{classification of test queries}
This paragraph describes the process for identifying subgroups of test queries with different relation patterns. We first mined rules from the triples-only dataset NELL995 \cite{NELL995} using the rule mining tool AMIE \cite{AMIE}. The rules that are significantly supported by a large amount of data and have body coverages greater than 0.2 are selected. These rules are then categorized into four types: symmetry, inversion, composition, and other. Each category includes a list of relations that encompass relation patterns. Using the selected relations, the test dataset of the logical query dataset NELL \cite{BetaE} is traversed, and queries are classified into five subgroups: symmetry, inversion, composition, joint, and other. A query is classified into a subgroup based on the presence of at least one relation from the corresponding relation subgroup. The joint subgroup includes queries that involve all three relation patterns, while the other subgroup does not include any of these patterns. 


\section{Model Robustness Check}
In this section, we check the model robustness of AConE by running AConE 10 times with different random seeds. The mean performance and standard deviations are reported in Table \ref{EPFOL(sd)}. The slight variances in the results indicate that AConE is robust to the different initializations of model parameters and our reported improvements are not due to randomness.



\section{Intersection}%
\label{sec:Intersection}

\begin{equation}
\begin{split}
    [\embedding{x};\embedding{y}] &= \sum_{k=1}^{n} [\embedding{a_k} \circ \cos(\AxAngle[k]);\embedding{a_k} \circ \sin(\AxAngle[k])],\\
    \AxAngle' &= \operatorname{Arg}(\embedding{x},\embedding{y}),
\end{split}
\end{equation}
where $\AxAngle[k]$ is the aperture angle of cone $\embedding{q_k}$, $\cos$ and $\sin$ are the element-wise cosine and sine functions, $\operatorname{Arg}$ computes the argument given $\embedding{x}$ and $\embedding{y}$, and  $\embedding{a_k} \in \Real^d$ are attention weights such that 
\begin{equation}
  \VectorComponent{\embedding{a_k}}{j} =
  \frac{
    \exp([\MLP([
      \VectorComponent{\AxAngle}{k} - \frac{\VectorComponent{\ApAngle}{k}}{2};\;
      \pmb{\theta}_{k,ax} + \pmb{\theta}_{k,ap/2}])]_{k})}{\sum_{m=1}^{n}\text{exp}([\MLP([\pmb{\theta}_{m,ax} - \pmb{\theta}_{m,ap/2};\pmb{\theta}_{m,ax} + \pmb{\theta}_{m,ap/2}])]_{j})}, 
\end{equation}
where \textbf{MLP} : $\mathbb{R}^{2d} \rightarrow \mathbb{R}^{d}$ is a multi-layer perceptron network, [$\cdot$;$\cdot$] is the concatenation of two vectors.

\paragraph{CardMin($\cdot$)} predicts the aperture $\pmb{\theta}_{ap}^{'}$ of the intersection set such that $[\pmb{\theta}_{ap}^{'}]_{i}$ should be no larger than any $\pmb{\theta}_{j,ap}^{i}$, since the intersection set is the subset of all input entity sets.
\begin{equation}
    [\theta_{ap}^{'}]_{i} = \text{min}\{\theta_{1,ap}^{i},\dots,\theta_{n,ap}^{i}\}\cdot\sigma([\textbf{DeepSets}(\{(\pmb{\theta}_{j,ax},\pmb{\theta}_{j,ap})\}_{j=1}^{n})]_{i})
\end{equation}
where \textbf{DeepSets}$(\{(\pmb{\theta}_{j,ax}, \pmb{\theta}_{j,ap})\}_{j=1}^{n})$ \cite{deepsets} is given by
\begin{equation}
    \textbf{MLP}(\frac{1}{n}\sum_{j=1}^{n}\textbf{MLP}([\pmb{\theta}_{j,ax} - \pmb{\theta}_{j,ap/2};\pmb{\theta}_{j,ax} + \pmb{\theta}_{j,ap/2}])).
\end{equation}


%%% Local Variables:
%%% TeX-master: "../main.tex"
%%% ispell-local-dictionary: "american"
%%% End:
